Revisiting Hierarchical Text Classification: Inference and Metrics

Hierarchical text classification (HTC) is the task of assigning labels to a text within a structured space organized as a hierarchy. Recent works treat HTC as a conventional multilabel classification problem, therefore evaluating it as such. We instead propose to evaluate models based on specifically designed hierarchical metrics and we demonstrate the intricacy of metric choice and prediction inference method. We introduce a new challenging dataset and we evaluate fairly, recent sophisticated models, comparing them with a range of simple but strong baselines, including a new theoretically motivated loss. Finally, we show that those baselines are very often competitive with the latest models. This highlights the importance of carefully considering the evaluation methodology when proposing new methods for HTC. Code implementation and dataset are available at \url{https://github.com/RomanPlaud/revisitingHTC}.

==> 3.problem.tex <==
\section{Problem definition}

Hierarchical Text classification (HTC) is a subtask of text classification which consists in assigning an input text $x \in \mathcal{X}$ to a set of labels $Y \subset \mathcal{Y}$, where the label space $\mathcal{Y}$ exhibits parent/child relations. We call hierarchy the undirected graph $\mathcal{H} = (\mathcal{Y}, \mathcal{E})$, where  $\mathcal{E} \subset \mathcal{Y}^2$ is the set of undirected edges, which goes from a parent to its children, and conversely. We restrain our study to the case where $\mathcal{H}$ is a tree. \\
We follow the notations introduced by \citet{NEURIPS2022_727855c3} and call $\mathbf{r} \in \mathcal{Y}$ the unique root node, $\mathcal{L}$ the set of leaf nodes. For a node $y \in \mathcal{Y}\backslash\{\mathbf{r}\}$ we denote $\pi(y)$ its unique parent, $\mathcal{C}(y) \subset \mathcal{Y}$ the set of its children and $\mathcal{A}(y)$ ($\mathcal{D}(y)$) the set of its ancestors (descendants). $\mathcal{A}(y)$ ($\mathcal{D}(y)$) is defined inclusively : $y\in\mathcal{A}(y)$ ($y\in\mathcal{D}(y)$). \\
A label set $Y$ of an input $x$ cannot be arbitrary : if $y\in Y$ then, due the parent relations, we necessarily observe that $\mathcal{A}(y)\subset Y$. 
% \mat{TODO: if I understand well, we do this restriction because it's needed for the metrics SP (and hF1 ?) - then we should say it before making that choice, I think.} 
An even more restrictive framework is the \textbf{Single-path leaf labels} setting where: 
\begin{enumerate}[itemsep=0.2em]
    \item $Y$ is a single path: $y_1, y_2 \in Y \Rightarrow y_1 \in \mathcal{A}(y_2) \text{ or } y_2 \in \mathcal{A}(y_1)$
    \item $Y\cap\mathcal{L} \ne \emptyset$
\end{enumerate}
In next sections, we will often refer to that framework, especially, to be able to (1) properly define the shortest path metric (2) give insights about inference methodology.
Again, as \citet{NEURIPS2022_727855c3}, we study methods that that maps an input text $x$ to a conditional distribution $\mathbb{P}(\cdot|x)$ over $\mathcal{Y}$, whose estimation is denoted $\hat{\mathrm{P}}(\cdot|x)$. 
% We furthermore identify key constraints on $\mathbb{P}$ : 
% \begin{itemize}
%     \item $\mathbf{r}$ shall be uninformative : $\mathbb{P}(\mathbf{r}|x) = 1$
%     \item $\mathbb{P}$ is \textbf{coherent} if :\\$\forall y\in\mathcal{Y},~ \mathbb{P}(y|x) \geq \underset{z\in\mathcal{C}(y)}{\sum}\mathbb{P}(z|x)$
%     \item $\mathbb{P}$ is \textbf{exhaustive} if :\\$\forall y\in\mathcal{Y},~ \mathbb{P}(y|x) = \underset{z\in\mathcal{C}(y)}{\sum}\mathbb{P}(z|x)$
% \end{itemize}

